Subjective Metrics-based Cloud Market Performance Prediction

This paper explores an effective machine learning approach to predict cloud market performance for cloud consumers, providers and investors based on social media. We identified a set of comprehensive subjective metrics that may affect cloud market performance via literature survey. We used a popular sentiment analysis technique to process customer reviews collected from social media. Cloud market revenue growth was selected as an indicator of cloud market performance. We considered the revenue growth of Amazon Web Services as the stakeholder of our experiments. Three machine learning models were selected: linear regression, artificial neural network, and support vector machine. These models were compared with a time series prediction model. We found that the set of subjective metrics is able to improve the prediction performance for all the models. The support vector machine showed the best prediction results compared to the other models.

==> intro <==
Numerous organisations are now choosing cloud computing as their technology of choice. Cloud computing can offer services on demand and on a per-usage payment basis, meaning cloud customers are not responsible for the maintenance of complex IT infrastructure. Cloud computing services are provided by vendors under the following categories: \textit{Software-as-a-Service (SaaS)}, \textit{Platform-as-a-Service (PaaS)}, and \textit{Infrastructure-as-a-Service (IaaS)} \cite{zhang2010cloud}. The focus of this paper is on the IaaS category. 

Many organisations utilise cloud services in their operations, while the cloud market comprises two types of participants: cloud customers and cloud investors or providers \cite{marston2011cloud}. Engagement in the market requires that both types of participant have a thorough comprehension of current trends in this specific market. Meanwhile, cloud providers and customers  must understand how various cloud services are performing. Sufficient knowledge of the cloud market allows the market participants to be aware of  opportunities, advantages, and risks associated with it. This can include knowledge of how the market is performing in terms of market competition, market growth, customer satisfaction, etc. \cite{mauboussin2012true}, which can all help in making informed decisions regarding the market. In fact, a comprehensive analysis of the market is of value to the cloud customer due to the long-term commitment involved. Such customers could be those who make IT decisions after determining the influence of emerging technologies.  They must understand how the market performs in terms of customer satisfaction, service quality, and many other factors before deciding to participate in the market. Investors also require information on market performance before making any decision to invest in stocks. In fact, many industry reports have been prepared by different organisations in relation to all the participants \cite{USDEP} \cite{451Research}. Most of these reports are concerned with the evaluation of cloud market size and growth as well as numerous other concerns. The reports tend to be produced after a thorough monitoring of the market.


The performance information provided by such reports are based on two types of metrics: objective metrics and subjective metrics. The objective metrics are based on actual facts without any individual bias. Examples of such metrics include market size and growth. According to 451Research \cite{451Research}, the collection of such data is frequently implemented through extensive market monitoring. Meanwhile, the subjective metrics are based on personal perceptions, opinions or feelings, an example being the information regarding the barriers to cloud adoption \cite{STATE}. Subjective measures are frequently obtained using industry surveys \cite{USDEP}\cite{RightScale}. Industries utilise either objective and subjective measures or a combination of both to produce industry reports. However, it is a challenge to apply objective metrics \cite{vij2016subjective} due to the information sensitivity, while it can be \textit{expensive}, \textit{time consuming} and \textit{less timely} to obtain the information required for objective performance. On the other hand, the gathering of subjective market information can be more practical, since the sharing of subjective evaluation information is preferred over objective evaluation information sharing \cite{vij2016subjective}. Market participants often tend to share similar information on \textit{social media}.


Numerous individuals are becoming increasingly involved in sharing their opinions on a variety of subjects in social media platforms. It has become increasingly popular in the recent years \cite{nepal2015trusting}. Specifically speaking, consumers express their complaints or their satisfaction with certain brands and services. It has been reported that one in three social media users prefer to use this outlet rather than contact the company by phone. Moreover, 50\% of social media users share their complaints/concerns about a service/brand at least once a month \cite{STATE}. Hence, social media can be viewed as a \textit{free and up-to-date} source of personal wisdom \cite{yu2012survey}.


How consumers perceive goods or services is likely to influence their purchase decisions \cite{ruiz2009drivers}. Thus, the subjective measures can be used to predict the future behaviour of the participants. With this subjective-based evaluation of market performance, a better comprehension of objectively-measured results can be gained. Any given customer review can include perceptions related to various areas of a product or service experience \cite{goh2013social}. In turn, these perceptions will influence the readers' perceptions and, subsequently, their purchase decisions \cite{mudambi2010research}. Here, perceptions related to risks, barriers and benefits can be particularly influential on a consumer's purchasing intention \cite{ruiz2009drivers}. Future behaviour can be predicted based on this intention to purchase \cite{shahabuddin2009forecasting}.
